Understanding Transformer from the Perspective of Associative Memory

In this paper, we share our reflections and insights on understanding Transformer architectures through the lens of associative memory--a classic psychological concept inspired by human cognition. We start with the basics of associative memory (think simple linear attention) and then dive into two dimensions: Memory Capacity: How much can a Transformer really remember, and how well? We introduce retrieval SNR to measure this and use a kernel perspective to mathematically reveal why Softmax Attention is so effective. We also show how FFNs can be seen as a type of associative memory, leading to insights on their design and potential improvements. Memory Update: How do these memories learn and evolve? We present a unified framework for understanding how different Transformer variants (like DeltaNet and Softmax Attention) update their "knowledge base". This leads us to tackle two provocative questions: 1. Are Transformers fundamentally limited in what they can express, and can we break these barriers? 2. If a Transformer had infinite context, would it become infinitely intelligent? We want to demystify Transformer architecture, offering a clearer understanding of existing designs. This exploration aims to provide fresh insights and spark new avenues for Transformer innovation.

==> sections/relatedwork.tex <==
\section{Related Work}

\subsection{Model Architecture}
Over the past many years, people have attempted various structures to enhance model's abilities from early RNN \cite{mikolov2010recurrent} and LSTM \cite{sundermeyer2012lstm} to the dominant Transformer \cite{vaswani2017attention} today. Transformer has quadratic complexity, and many efforts have been made to improve them \cite{peng2023rwkv,gu2023mamba,sun2023retentive,beck2024xlstm,qin2022cosformer}. Nevertheless, Transformers still has many excellent properties that cannot be replaced temporarily, especially their ability to retrieve information and adapt
to a form of dynamic sparsity \cite{jelassirepeat,alman2024fundamental,mousavi2025transformers}. Currently, popular language models \citep{achiam2023gpt,dubey2024llama,yang2024qwen2} still use Transformer as the main architecture and some works use a hybrid architecture \cite{ren2024samba,lieber2024jamba,li2025minimax}. Recently, there have been some studies that have shown that DeltaNet and some variants \cite{schlag2021linear,yang2024deltanet,yang2024gated,peng2025rwkv,siems2025deltaproduct} can overcome the complexity limitations of $\text{TC}^0$ where Transformer is located, resulting in higher expressiveness and achieving good performance in tasks such as state tracking \cite{grazzi2024unlocking,siems2025deltaproduct,merrill2024illusion}. Our paper aims to re-examine the properties of Transformer, enhance our understanding of Transformer, and make improvements to break through the expressive limitations of Transformer.

\subsection{Understanding Transformer} 
Since the popularity of Transformer \cite{vaswani2017transformer}, extensive research has also been conducted on their underlying machines. Some works analyzed its powerful approximation ability \cite{yun2019transformers, dong2021attention,kim2022pure}. There are also some tasks aimed at understanding the dynamics of model training \cite{makkuva2024local,bietti2023birth,tianjoma} and interpretability \cite{chefer2021transformer,lindner2023tracr,lindsey2025biology,zhu2024physics_llm}. With the development of large models, more and more understanding work focus on analyzing the contextual learning ability of transformers \cite{garg2022can,li2023transformers,olsson2022context,elhage2021mathematical,elhage2022solu,elhage2022superposition,wang2025r}. An important aspect for understanding the behavior of large models is the associative memory \cite{niu2024beyond,kang2025lm2,behrouz2024titans,wang2025test_time_regression}, and we start our work from here. We want to understand the transformer from the perspective of associative memory, and draw inspiration from it to guide the design of new models. 
